Multipar-T: Multiparty-Transformer for Capturing Contingent Behaviors in Group Conversations

As we move closer to real-world AI systems, AI agents must be able to deal with multiparty (group) conversations. Recognizing and interpreting multiparty behaviors is challenging, as the system must recognize individual behavioral cues, deal with the complexity of multiple streams of data from multiple people, and recognize the subtle contingent social exchanges that take place amongst group members. To tackle this challenge, we propose the Multiparty-Transformer (Multipar-T), a transformer model for multiparty behavior modeling. The core component of our proposed approach is the Crossperson Attention, which is specifically designed to detect contingent behavior between pairs of people. We verify the effectiveness of Multipar-T on a publicly available video-based group engagement detection benchmark, where it outperforms state-of-the-art approaches in average F-1 scores by 5.2% and individual class F-1 scores by up to 10.0%. Through qualitative analysis, we show that our Crossperson Attention module is able to discover contingent behavior.

==> z89_more_qual_fig.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/qual_2.pdf}
    \caption{(a) \modelss Cross-person Attention weights from $t=336s$ for group $S02$. \modelshorts has discovered that $self$’s behavior from timestep 4-10 is contingent on $other$’s behavior in timestep 10 – 35 (smile). }

\end{figure*}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/qual_3.pdf}
    \caption{(a) \modelss Cross-person Attention weights from $t=96s$ for group $S08$. \modelshorts has discovered that $self$’s behavior from timestep 10-35 is contingent on $other$’s behavior in timestep 4-7. }

\end{figure*}

==> z90_attn_weights.tex <==
\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/attn_weights_1.pdf}

\end{figure*}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/attn_weights_2.pdf}

\end{figure*}

\begin{figure*}[!ht]
    \centering
    \includegraphics[width=0.9\textwidth]{figs/attn_weights_3.pdf}
    \caption{Diverse \modelss Cross-person Attention weights, we see that our model captures non-uniform and interesting attention weights to capture behavior interactions across pairs of people.}

\end{figure*}

==> z94_transformer_fig.tex <==
\begin{figure*}[t]
    \vspace{-0mm}
    \begin{center}
    \includegraphics[width=0.8\textwidth]{figs/transformer.pdf}
    \caption{crossperson attention fig}
    \label{fig:fullmodel}
    \end{center}
\end{figure*}

==> z95_model_fig.tex <==
\begin{figure}[t]
    \vspace{-0mm}
    \begin{center}
    \includegraphics[width=1.1\columnwidth]{figs/model.pdf}
    \caption{(a) Diagram of our \cpas module, which takes in pairs of behavioral features and automatically searches for the contingencies between behaviors. (b) Diagram of our Cross-Person Transformer Module. (c) Diagram of our overarching model: \modelss, that takes in all unique pairs of behavioral features, (Person 1), and contextualizes pairwise contingent behavior with respect to the target person. then is passed through an temporal group classifier  }
    \label{fig:model}
    \end{center}
\end{figure}
